An eigenspace approach to isotypic projections for data on binary trees

The classical Fourier transform is, in essence, a way to take data and extract components (in the form of complex exponentials) which are invariant under cyclic shifts. We consider a case in which the components must instead be invariant under automorphisms of a binary tree. We present a technique by which a slightly relaxed form of the generalized Fourier transform in this case can eventually be computed using only simple tools from linear algebra, which has possible advantages in computational efficiency.

==> math.tex <==
% A -*- latex -*- file.

% List of commands I'm going to use in Real Analysis (and maybe beyond...)

\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}

% Pretty symbols for sets I will use a lot.

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

% For vectors.
\renewcommand{\vec}[1]{\mathbf{#1}}

% Nice way to show problems.

\newcommand{\generalproblem}[1]{\subsection*{#1}}

\newcommand{\problem}[1]{\generalproblem{Problem #1}}

% Theorems, lemmae, etc.  Not numbered.

\theoremstyle{plain} % Heading in bold, text in italics.
\newtheorem*{theorem}{Theorem}
\newtheorem*{corollary}{Corollary}
\newtheorem*{lemma}{Lemma}
\newtheorem*{claim}{Claim}
\newtheorem*{proposition}{Proposition}
\newtheorem*{problemstatement}{Problem} % \problem is taken :)
\newtheorem*{question}{Question}

% Numbered variant.
\newtheorem{lemmaN}{Lemma}
\newtheorem{theoremN}{Theorem}
\newtheorem{propositionN}{Proposition}
\newtheorem{problemstatementN}{Problem}

\theoremstyle{definition} % Bold header, roman text
\newtheorem*{definition}{Definition}
\newtheorem*{conjecture}{Conjecture}
\newtheorem*{example}{Example}

\theoremstyle{remark} % Italic header, roman text
\newtheorem*{remark}{Remark}
\newtheorem*{note}{Note}
\newtheorem*{case}{Case}
\newtheorem*{answer}{Answer}
\newtheorem*{solution}{Solution}

\newcommand{\contradiction}{$\Rightarrow \Leftarrow$}

\newcommand{\divides}{|}
% \newcommand{\ndivides}{\nmid}

% Handy functions.

% The \lvert and \rvert recommended by ams don't scale.
\newcommand{\abs}[1]{\left| #1 \right|}
%\newcommand{\norm}[1]{\abs{#1}}
\newcommand{\conj}[1]{\overline{#1}}
% complement a set
\newcommand{\comp}[1]{#1^C}

\newcommand{\diam}{\mathop{\rm diam}\nolimits}

% For use in set-builder notation.
\newcommand{\where}[1]{\left| \, #1 \right.}

% Ick.  \bar is too short, but \overline is a bit too long.  But at
% least it's more obvious.
%\newcommand{\closure}[1]{\bar{#1}}
\newcommand{\closure}[1]{\overline{#1}}

\newcommand{\interior}[1]{#1^\circ}

% These don't scale either, but I haven't found an alternative yet.
\newcommand{\norm}[1]{\lVert #1 \rVert }

% The built-in commands are just R and I in a funny font.  I'm
% not sure I like it, so here are alternatives.
%\renewcommand{\Re}{\mathrm{Re}}
%\renewcommand{\Im}{\mathrm{Im}}

\newcommand{\qe}{\overset{?}=}

\newcommand{\fixme}[1]{\marginpar{\fbox{Fix me! #1}}}

\hyphenation{ei-gen-space ei-gen-spac-es ei-gen-val-ue ei-gen-val-ues
  ei-gen-vec-tor ei-gen-vec-tors}


==> reps.tex <==
% -*- latex -*-

%%% This file has been expunged.

